Is Next Token Prediction Sufficient for GPT? Exploration on Code Logic Comprehension

Large language models (LLMs) has experienced exponential growth, they demonstrate remarkable performance across various tasks. Notwithstanding, contemporary research primarily centers on enhancing the size and quality of pretraining data, still utilizing the next token prediction task on autoregressive transformer model structure. The efficacy of this task in truly facilitating the model's comprehension of code logic remains questionable, we speculate that it still interprets code as mere text, while human emphasizes the underlying logical knowledge. In order to prove it, we introduce a new task, "Logically Equivalent Code Selection," which necessitates the selection of logically equivalent code from a candidate set, given a query code. Our experimental findings indicate that current LLMs underperform in this task, since they understand code by unordered bag of keywords. To ameliorate their performance, we propose an advanced pretraining task, "Next Token Prediction+". This task aims to modify the sentence embedding distribution of the LLM without sacrificing its generative capabilities. Our experimental results reveal that following this pretraining, both Code Llama and StarCoder, the prevalent code domain pretraining models, display significant improvements on our logically equivalent code selection task and the code completion task.

==> tables/Code_Completion_Task_Results.tex <==
\captionsetup[table]{font={small}}
\begin{table*}[ht]
\centering 
\begin{adjustbox}{width=\linewidth}
\resizebox{0.8\linewidth}{!}{%  
\begin{tabular}{c|c|c|c|c|c|c}  
\hline  
Model & \multicolumn{3}{c|}{PY150} & \multicolumn{3}{c}{Java Corpus} \\  
\hline  
Subtask & token-level & \multicolumn{2}{c|}{line-level} & token-level & \multicolumn{2}{c}{line-level} \\  
\hline 
Metric & Acc & EM & ES & Acc & EM & ES \\
\hline
Code Llama7b & 83.57 & 50.79 & 75.26 & 83.11 & 40.07 & 73.21 \\
+pretrain & 86.51 & 52.14 & 77.31 & 86.69 & 42.61 & 76.53 \\
Code Llama13b & - & - & - & - & - & - \\
+pretrain & - & - & - & 88.05 & 40.42 & 75.38 \\
Starcoder15b & 85.9 & 54.27 & 78.17 & 83.17 & 40.18 & 74.22 \\
+pretrain & 87.23 & 56.13 & 81.16 & 84.49 & 43.05 & 76.93\\
\hline 
CodeGPT-adapted & 76.60 & 42.37 & 71.59 & 77.73 & 30.60 & 63.45 \\
CodeT5+ 770M & - & 44.86 & 74.22 & - & 37.90 & 72.25 \\
PyCoder & 76.93 & 43.91 & 71.74 & - & - & - \\
\hline  
\end{tabular}%  
}   
\end{adjustbox}

\caption{\raggedright {\textbf{Compare the model performance in Code Logic Equivalence Determination Task.}  } }
\label{table:Code_Completion_Task_Results}

\end{table*}

==> tables/embedding_similar_table.tex <==
\captionsetup[table]{font={small}}
\begin{table*}[ht]

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|cccccc}
\hline
\textbf{Model} & $D_{Pos}>D_{Neg}$ & $D_{Obf}>D_{Neg}$ & $D_{Pos}>D_{LSh}$ & $D_{Pos}>D_{TSh}$ & $D_{Pos}>D_{KDe}$ & $D_{Pos}>D_{SDe}$ \\
\hline
Code Llama 7B & {45.4\%} & {8.4\%} & {19.2\%} & {87.1\%} & {89.5\%} & {72.5\%} \\
Code Llama 13B & {66.4\%} & {11.8\%} & {26.1\%} & {99.7\%} & {96.3\%} & {87.7\%}\\
StarCoder Base & {67.2\%} & {13.1\%} & {44.7\%} & {99.8\%} & {96.5\%} & {85.9\%}\\
\hline
text-embedding-ada-002 & {94.4\%} & {34.0\%} & {67.6\%} & {99.5\%} & {98.1\%} & {98.7\%}\\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{\raggedright {\textbf{Embedding Similarities Analysis.} We calculated the distances between positive code, negative code, obfused code, line shuffle code, token shuffle code, keyword delete code, symbol delete code and origin code in embedding space respectively (expressed as $D_{Pos}$, $D_{Neg}$, $D_{Obf}$, $D_{LSh}$, $D_{TSh}$, $D_{KDe}$, $D_{SDe}$). We selected 7 scenarios that are challenging for large language models and calculated their ratio to alignment with human intuition. We also selected OpenAI’s most powerful sentence vector representation model, text-embedding-ada-002, for comparison.}}
\label{table:embedding_similar_table}

\end{table*}

==> tables/pretrained_prompt_qa_similar_table.tex <==
\captionsetup[table]{font={small}}
\begin{table*}[ht]

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|cccccc}
\hline
\textbf{Model} & $Acc(Pos>Neg)$ & $Acc(Obf>Neg)$ & $Acc(Pos>LSh)$ & $Acc(Pos>TSh)$ & $Acc(Pos>KDe)$ & $Acc(Pos>SDe)$ \\
\hline
Code Llama 7B & {0} & {0} & {0} & {0} & {0} & {0} \\
Code Llama 13B & {66.4\%} & {1.8\%} & {26.1\%} & {99.7\%} & {0} & {0}\\
StarCoder Base & {67.2\%} & {3.1\%} & {44.7\%} & {99.8\%} & {0} & {0}\\
StarCoder & {0} & {0} & {0} & {0} & {0} & {0}\\
\hline
Code Llama 7B + Pretrain & {0} & {0} & {0} & {0} & {0} & {0} \\
Code Llama 13B + Pretrain & {66.4\%} & {1.8\%} & {26.1\%} & {99.7\%} & {0} & {0}\\
StarCoder Base + Pretrain & {67.2\%} & {3.1\%} & {44.7\%} & {99.8\%} & {0} & {0}\\
StarCoder + Pretrain & {0} & {0} & {0} & {0} & {0} & {0}\\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{\raggedright {\textbf{Compare the model performance in Prompt Question-Answer Similarities Analysis task.}}}
\label{table:pretrained_prompt_qa_similar_table}

\end{table*}

==> tables/prompt_qa_similar_table.tex <==
\captionsetup[table]{font={small}}
\begin{table*}[ht]

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|cccccc}
\hline
\textbf{Model} & $Acc(Pos>Neg)$ & $Acc(Obf>Neg)$ & $Acc(Pos>LSh)$ & $Acc(Pos>TSh)$ & $Acc(Pos>KDe)$ & $Acc(Pos>SDe)$ \\
\hline
Code Llama 7B & {0} & {0} & {0} & {0} & {0} & {0} \\
Code Llama 13B & {66.4\%} & {1.8\%} & {26.1\%} & {99.7\%} & {0} & {0}\\
StarCoder Base & {45.3\%} & {50.4\%} & {43.9\%} & {56.7\%} & {0} & {0}\\
\hline
gpt-3.5-turbo & {85.4\%} & {95.5\%} & {43.2\%} & {76.2\%} & {98.9\%} & {97.0\%}\\
gpt-4 & {86.2\%} & {97.6\%} & {43.8\%} & {80.5\%} & {98.3\%} & {97.4\%}\\
\bottomrule
\end{tabular}
\end{adjustbox}

\caption{\raggedright {\textbf{Prompt Question-Answer Similarities Analysis.} We employ a question-and-answer template to evaluate which option code the model deems to be more pertinent to the original code. The term $Acc(Pos>Neg)$ signifies the accuracy of the model in selecting the appropriate option of positive code when presented with two candidates, namely, the positive and negative codes. The remaining cases can be inferred similarly. We have selected OpenAI’s gpt-3.5-turobo and gpt-4 models as benchmarks for this analysis.}}
\label{table:prompt_qa_similar_table}

\end{table*}

==> unused.tex <==
In recent years, Large Language Models (LLMs) have gained significant prominence and demonstrated remarkable effectiveness across diverse applications \citep{openai-2023-gpt4, yang-2023-harnessing}. 
These models harness the power of extensive pre-training on vast internet datasets, followed by fine-tuning with task-specific instruction data, leading to state-of-the-art zero-shot or few-shot performance on a wide array of tasks. 
This trend is especially notable in the realm of code comprehension and generation, where Code LLMs have emerged as promising solutions to tackle code-related challenges.


